UrbanLoco: A Full Sensor Suite Dataset for Mapping and Localization in Urban Scenes

Mapping and localization is a critical module of autonomous driving, and significant achievements have been reached in this field. Beyond Global Navigation Satellite System (GNSS), research in point cloud registration, visual feature matching, and inertia navigation has greatly enhanced the accuracy and robustness of mapping and localization in different scenarios. However, highly urbanized scenes are still challenging: LIDAR- and camera-based methods perform poorly with numerous dynamic objects; the GNSS-based solutions experience signal loss and multipath problems; the inertia measurement units (IMU) suffer from drifting. Unfortunately, current public datasets either do not adequately address this urban challenge or do not provide enough sensor information related to mapping and localization. Here we present UrbanLoco: a mapping/localization dataset collected in highly-urbanized environments with a full sensor-suite. The dataset includes 13 trajectories collected in San Francisco and Hong Kong, covering a total length of over 40 kilometers. Our dataset includes a wide variety of urban terrains: urban canyons, bridges, tunnels, sharp turns, etc. More importantly, our dataset includes information from LIDAR, cameras, IMU, and GNSS receivers. Now the dataset is publicly available through the link in the footnote. Dataset Link: https://advdataset2019.wixsite.com/urbanloco.

==> trash-can.tex <==

\subsection{Data Format}
This section introduces the data format in this dataset. The data is collected through ROS \cite{ROS}, in separated ROS bags to satisfy most SLAM algorithm designs. The ROS messages are lined up in UNIX time stamps. Each sensor is associated with one or multiple topics shown below. 

\begin{description}
  \item[$\bullet$ LIDAR] The 3D LIDAR data was recorded using standard PointCloud2 ROS message. The message contains both geometry and intensity information of the ranging points. One could refer to \textit{/velodyne\_point} or \textit{/rslidar\_points} topic in the ROS bag file;
  \item[$\bullet$ Camera] The camera information are stored as a compressed image message in the ROS bag. One could refer to \textit{/camera\_array/cam0/image\_raw/compressed} topics etc.;
  \item[$\bullet$ IMU] The acceleration/velocity message is stored in the \textit{/imu\_raw} topic as a ROS sensor\_msgs/IMU. We also provided the magnetic angle sensing from \textit{/mti/sensor/magnetic};
  \item[$\bullet$ GNSS] All topics associated with Ublox is published under \textit{/ublox} topics. The message is published as a navsat sentence;
  \item[$\bullet$ Ground Truth] For the 20Hz localization ground truth, the user should refer to \textit{/novatel\_data/inspvax} topic. \textit{/novatel\_data/inspvax} contains a custom message type built by Novatel, but it is supported and maintained on ROS.
\end{description}


